Preferences Evolve And So Should Your Bandits: Bandits with Evolving States for Online Platforms

We propose a model for learning with bandit feedback while accounting for deterministically evolving and unobservable states that we call Bandits with Deterministically Evolving States ($B$-$DES$). The workhorse applications of our model are learning for recommendation systems and learning for online ads. In both cases, the reward that the algorithm obtains at each round is a function of the short-term reward of the action chosen and how "healthy" the system is (i.e., as measured by its state). For example, in recommendation systems, the reward that the platform obtains from a user's engagement with a particular type of content depends not only on the inherent features of the specific content, but also on how the user's preferences have evolved as a result of interacting with other types of content on the platform. Our general model accounts for the different rate $\lambda \in [0,1]$ at which the state evolves (e.g., how fast a user's preferences shift as a result of previous content consumption) and encompasses standard multi-armed bandits as a special case. The goal of the algorithm is to minimize a notion of regret against the best-fixed sequence of arms pulled, which is significantly harder to attain compared to standard benchmark of the best-fixed action in hindsight. We present online learning algorithms for any possible value of the evolution rate $\lambda$ and we show the robustness of our results to various model misspecifications.

==> relaxation.tex <==
\section{Relaxation: Dynamic Programming with Approximate Rewards}\label{sec:DP-relax}

In this section, we present a relaxation for the problem, where for each arm the learner has \emph{estimates of bounded error} about $(r_i, b_i)$. Then, we show the efficiency (compared to $\OPT$) of a Dynamic Programming approach that takes as input these estimates and outputs a sequence of arms. The proofs of this section can be found in Appendix~\ref{app:DP-relax}.

We begin by presenting the closed form solution for the state at each $t$. This is useful for designing the dynamic program.
%~\ref{app:DP-relax}.

\begin{lemma}\label{lem:state-closed-form}
Let $\ALG$ be an algorithm pulling arm $I_t$ at round $t$. The closed form solution for computing the state at each round is: 
\begin{equation}\label{eq:qt-closed-form}
q_{t+1} \left( H_{1:t}^\ALG \right) = (1-\lambda)^t \cdot q_0 + \lambda \cdot \sum_{s = 0}^{t-1} (1 - \lambda)^{t-1-s} \cdot b_{I_s}
\end{equation}
\end{lemma}


This closed-form solution for the state is important, since it allows us to directly decompose $q_{t+1}(H_t^\ALG)$ to the baseline rewards of the arms pulled so far. This is helpful because, as we argue below, we do not need to have full knowledge of the exact baseline rewards; instead, good approximations are enough to give us a solution that is close to the $\OPT$. 

\begin{lemma}\label{lem:approx-DP}
Let $\hDP$ denote the expected reward of the solution returned by a dynamic programming algorithm with inputs $(\hr_i, \hb_i)_{i \in [K]}$, where $|\hr_i - r_i| \leq \delta$ and $|\hb_i - b_i| \leq \delta$. %This dynamic programming algorithm outputs a policy for choosing an arm at each round. 
Then, $\hDP \geq \OPT - \delta T$.
\end{lemma}


The dynamic programming algorithm that uses $(\hr_i, \hb_i)_{i \in [K]}$ as inputs returns a policy for choosing an arm in each round. Notice that our problem here has a knapsack-style structure; in order to construct the dynamic programming algorithm we need to do the following. For each $T$, associate for each sequence $(i_1, \dots, i_T)$ both the total reward $\rho_T$ and the final state $q_T$. This means that for each $t$, we have a list of possible $(\rho_t, q_t)$. Let us call this list $F_t = \{(\rho_t, q_t)\}_t$. Then, one can construct $F_{t+1}$ from $F_t$ as $F_{t+1} = \{(\rho + \hr_j \cdot q, (1-\lambda) \cdot q + \lambda \cdot \hb_j)\}$ for tuple $(\rho, q) \in F_t$ and $j \in [K]$. Indeed, similar to the dynamic programming in knapsack, $F_t$ can grow exponentially large in $T$. However, one can round to multiples of $\epsilon$, remove dominated tuple components, and end up with at most $1/\epsilon$ points in each $F_t$. This approach gives a PTAS for the problem (see e.g.,~\cite{williamson2011design})  


Below, we use the dynamic programming algorithm as follows. First, we obtain the estimates $(\hr_i, \hb_i)_{i \in [K]}$ if there exists a \emph{known} ``replenishing'' arm $i_R$, for which it holds that $b_{i_R} \in [1 - 2\eps, 1-\eps]$. Second, we show a method for relaxing this assumption, while still obtaining meaningful estimates. When the estimates are obtained, the algorithm feeds them to the dynamic programming subroutine. Due to Lemma~\ref{lem:approx-DP}, if the estimates are good enough, the algorithm will compute a solution.
